Substitute Teacher Networks: Learning with Almost No Supervision

Learning through experience is time-consuming, inefficient and often bad for your cortisol levels. To address this problem, a number of recently proposed teacher-student methods have demonstrated the benefits of private tuition, in which a single model learns from an ensemble of more experienced tutors. Unfortunately, the cost of such supervision restricts good representations to a privileged minority. Unsupervised learning can be used to lower tuition fees, but runs the risk of producing networks that require extracurriculum learning to strengthen their CVs and create their own LinkedIn profiles. Inspired by the logo on a promotional stress ball at a local recruitment fair, we make the following three contributions. First, we propose a novel almost no supervision training algorithm that is effective, yet highly scalable in the number of student networks being supervised, ensuring that education remains affordable. Second, we demonstrate our approach on a typical use case: learning to bake, developing a method that tastily surpasses the current state of the art. Finally, we provide a rigorous quantitive analysis of our method, proving that we have access to a calculator. Our work calls into question the long-held dogma that life is the best teacher.

==> biographies.tex <==
\section*{Authors' Biographies}
%TODO

==> iclr2016_conference.tex <==
@article{croton,
  title={How to bake the perfect croton},
  author="{Philolaus of Croton}",
  journal={Greek Journal of Fine, Fine Cuisine},
  year={421 BC}
}

@article{sutton1999between,
  title={Between MDPs and semi-MDPs: A framework for temporal abstraction in reinforcement learning},
  author={Sutton, Richard S and Precup, Doina and Singh, Satinder},
  journal={Artificial intelligence},
  volume={112},
  number={1-2},
  pages={181--211},
  year={1999},
  publisher={Elsevier}
}

@book{oksendalSDE,
    author = {{\O}ksendal, Bernt},
    edition = {6th},
    howpublished = {Paperback},
    isbn = {3540047581},
    keywords = {probability, statistics},
    month = jan,
    posted-at = {2007-09-27 18:06:09},
    priority = {2},
    publisher = {Springer},
    title = {{Stochastic Differential Equations: An Introduction with Applications (Universitext)}},
    url = {http://www.amazon.com/exec/obidos/redirect?tag=citeulike07-20\&path=ASIN/3540047581},
    year = {2014}
}

@inproceedings{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  booktitle={Neural Information Processing Systems, conference on},
  year={2015}
}

@inproceedings{LeCun16,
  title={{Keynote Address: Predictive Learning}},
  author={LeCun, Yann},
  journal={Advances in neural information processing systems},
  year={2016},
} (edited)

@inproceedings{Abbeel17,
  title={{Keynote Address: Deep Learning for Robotics}},
  author={Pieter Abbeel},
  journal={Advances in neural information processing systems},
  year={2017},
}
@inproceedings{rahimi,
  title={{Test of Time Award Ceremony}},
  author={Ali Rahimi},
  journal={Advances in neural information processing systems},
  year={2017},
}

@misc{amazon,
    author = {Amazon},
    title = {Details redacted due to active {NDA} clause.},
}

@article{li2016hyperband,
  title={Hyperband: A novel bandit-based approach to hyperparameter optimization},
  author={Li, Lisha and Jamieson, Kevin and DeSalvo, Giulia and Rostamizadeh, Afshin and Talwalkar, Ameet},
  journal={arXiv preprint arXiv:1603.06560},
  year={2016}
}

@inproceedings{snoek2012practical,
  title={Practical bayesian optimization of machine learning algorithms},
  author={Snoek, Jasper and Larochelle, Hugo and Adams, Ryan P},
  booktitle={Advances in neural information processing systems},
  pages={2951--2959},
  year={2012}
}


@article{searle1980minds,
  title={Minds, brains, and programs},
  author={Searle, John R},
  journal={Behavioral and brain sciences},
  volume={3},
  number={3},
  pages={417--424},
  year={1980},
  publisher={Cambridge University Press}
}



@article{scott2006jenga,
  title={Jenga},
  author={Scott, Leslie},
  journal={Board game, Hasbro: Pawtucket, RI},
  year={2006}
}

@article{piaget1970piaget,
  title={Piaget's theory},
  author={Piaget, Jean},
  year={1970},
  publisher={Wiley New York}
}

@article{crowley2017moonshine,
  title={Moonshine: Distilling with Cheap Convolutions},
  author={Crowley, Elliot J and Gray, Gavin and Storkey, Amos},
  journal={arXiv preprint arXiv:1711.02613},
  year={2017}
}

@inproceedings{vedaldi2015matconvnet,
  title={Matconvnet: Convolutional neural networks for matlab},
  author={Vedaldi, Andrea and Lenc, Karel},
  booktitle={Proceedings of the 23rd ACM international conference on Multimedia},
  pages={689--692},
  year={2015},
  organization={ACM}
}

@misc{fouhey2012kardashian,
  title={The Kardashian Kernel},
  author={Fouhey, David F and Maturana, Daniel},
  year={2012},
  publisher={SIGBOVIK}
}

@inproceedings{timberlake,
  title={{Filthy (Official Music Video)}},
  author={Timberlake, Justin},
  booktitle={{Pan-Asian Deep Learning Conference}},
  year={2028},
  note={Kuala Lumpur, Malaysia}
}

@inproceedings{albanie29,
  title={{How I learned to stop worrying and love the machines (Official Music Video)}},
  author={{JT-9000}},
  booktitle={{British Machine Vision Conference (BMVC)}},
  year={2029},
  note={West Butterwick, just 7 miles from Scunthorpe, England}
}

@inproceedings{fouhey13, 
 title={{You Only Learn Once - A Stochastically Weighted AGGRegation approach to online regret minimization}},
 author={Maturana, Daniel and Fouhey, David},
 booktitle={Proceedings of the 7th ACH SIGBOVIK Special Interest Group on Harry Quechua Bovik.},
 year={2013}, 
}

@article{albanie2017stopping,
  title={Stopping GAN Violence: Generative Unadversarial Networks},
  author={Albanie, Samuel and Ehrhardt, S{\'e}bastien and Henriques, Jo{\~a}o F},
  journal={Proceedings of the 11th ACH SIGBOVIK Special Interest Group on Harry Quechua Bovik.},
  year={2017}
}

@article{albanie2019,
  title={Defeating Google Scholar with citations into the future},
  author={Albanie, Samuel and Ehrhardt, S{\'e}bastien and James Thewlis and Henriques, Jo{\~a}o F},
  journal={Proceedings of the 13th ACH SIGBOVIK Special Interest Group on Harry Quechua Bovik.},
  year={2019}
}

@inproceedings{bucilua2006model,
  title={Model compression},
  author={Bucilua, Cristian and Caruana, Rich and Niculescu-Mizil, Alexandru},
  booktitle={Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={535--541},
  year={2006},
  organization={ACM}
}

@article{crowley2017moonshine,
  title={Moonshine: Distilling with Cheap Convolutions},
  author={Crowley, Elliot J and Gray, Gavin and Storkey, Amos},
  journal={arXiv preprint arXiv:1711.02613},
  year={2017}
}

@book{stiller2004zoolander,
  title={Zoolander},
  author={Zoolander, Derek et. al},
  year={2004},
  publisher={Paramount Pictures}
}

@inproceedings{eslami2016attend,
  title={Attend, infer, repeat: Fast scene understanding with generative models},
  author={Eslami, SM Ali and Heess, Nicolas and Weber, Theophane and Tassa, Yuval and Szepesvari, David and Hinton, Geoffrey E and others},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3225--3233},
  year={2016}
}

@article{jaderberg2016decoupled,
  title={Decoupled neural interfaces using synthetic gradients},
  author={Jaderberg, Max and Czarnecki, Wojciech Marian and Osindero, Simon and Vinyals, Oriol and Graves, Alex and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1608.05343},
  year={2016}
}

@article{amari1998natural,
  title={Natural gradient works efficiently in learning},
  author={Amari, Shun-Ichi},
  journal={Neural computation},
  volume={10},
  number={2},
  pages={251--276},
  year={1998},
  publisher={MIT Press}
}


@article{rusu2015policy,
  title={Policy distillation},
  author={Rusu, Andrei A and Colmenarejo, Sergio Gomez and Gulcehre, Caglar and Desjardins, Guillaume and Kirkpatrick, James and Pascanu, Razvan and Mnih, Volodymyr and Kavukcuoglu, Koray and Hadsell, Raia},
  journal={arXiv preprint arXiv:1511.06295},
  year={2015}
}

@inproceedings{parisotto16_actormimic,
  author    = {Emilio Parisotto and Jimmy Ba and Ruslan Salakhutdinov},
  title     = {Actor-Mimic: Deep Multitask and Transfer Reinforcement Learning},
  booktitle = {ICLR},
  year      = {2016}
}v

@article{schmitt2018kickstarting,
  title={Kickstarting Deep Reinforcement Learning},
  author={Schmitt, Simon and Hudson, Jonathan J and Zidek, Augustin and Osindero, Simon and Doersch, Carl and Czarnecki, Wojciech M and Leibo, Joel Z and Kuttler, Heinrich and Zisserman, Andrew and Simonyan, Karen and others},
  journal={arXiv preprint arXiv:1803.03835},
  year={2018}
}

	
@article{belagiannis2018anc,
  title={Adversarial Network Compression},
  author={Belagiannis, Vasileios  and Farshad, Azade and Galasso, Fabio},
  journal={arXiv preprint 	arXiv:1803.10750},
  year={2018}
}

@MISC{wolfram,
  author={Stephen Wolfram},
  title={What is Spacetime Really?},
  year={2015},
  note="\url{http://blog.stephenwolfram.com/2015/12/what-is-spacetime-really/}"
}

@inproceedings{xu2016ask,
  title={Ask, attend and answer: Exploring question-guided spatial attention for visual question answering},
  author={Xu, Huijuan and Saenko, Kate},
  booktitle={European Conference on Computer Vision},
  pages={451--466},
  year={2016},
  organization={Springer}
}

@inproceedings{arandjelovic2017look,
  title={Look, listen and learn},
  author={Arandjelovic, Relja and Zisserman, Andrew},
  booktitle={2017 IEEE International Conference on Computer Vision (ICCV)},
  pages={609--617},
  year={2017},
  organization={IEEE}
}

@article{redmon2018yoloV3,
  title={YOLOv3: An Incremental Improvement},
  author={Redmon,Joseph and Farhadi, Ali},
  howpublished = "\url{https://pjreddie.com/media/files/papers/YOLOv3.pdf}",
  year={2018},
}

@article{sims2003enron,
  title={Enron ethics (or: culture matters more than codes)},
  author={Sims, Ronald R and Brinkmann, Johannes},
  journal={Journal of Business ethics},
  volume={45},
  number={3},
  pages={243--256},
  year={2003},
  publisher={Springer}
}

@inproceedings{jegou2017one,
  title={The one hundred layers tiramisu: Fully convolutional densenets for semantic segmentation},
  author={J{\'e}gou, Simon and Drozdzal, Michal and Vazquez, David and Romero, Adriana and Bengio, Yoshua},
  booktitle={Computer Vision and Pattern Recognition Workshops (CVPRW), 2017 IEEE Conference on},
  pages={1175--1183},
  year={2017},
  organization={IEEE}
}

@article{wu2018gn,
  title={Group Normalization},
  author={Wu, Yuxin and He, Kaiming},
  journal={arXiv preprint arXiv:1803.08494},
  year={2018}
}

@article{ulyanov2016in,
  title={Instance normalization: The missing ingredient for fast stylization},
  author={Ulyanov, Dmitry and Vedaldi, Andrea and Lempitsky, Victor},
  journal={arXiv preprint arXiv:1607.08022},
  year={2016}
}

@article{ba2016layer,
  title={Layer normalization},
  author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  journal={arXiv preprint arXiv:1607.06450},
  year={2016}
}

@article{ioffe2015batch,
  title={Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  journal={arXiv preprint arXiv:1502.03167},
  year={2015}
}

@inproceedings{gupta2016cross,
  title={Cross modal distillation for supervision transfer},
  author={Gupta, Saurabh and Hoffman, Judy and Malik, Jitendra},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2016 IEEE Conference on},
  pages={2827--2836},
  year={2016},
  organization={IEEE},
}

@article{ardalanihave18,
  title={Have a Larger Cake and Eat it Faster Too: A Guideline to Train Larger Models Faster},
  author={Ardalani, Newsha and Hestness, Joel and Diamos, Gregory},
  year={2018},
  journal={SysML},  
}

@book{gilbert2009eat,
  title={Eat pray love: One woman's search for everything},
  author={Gilbert, Elizabeth},
  year={2009},
  publisher={Bloomsbury Publishing}
}

==> model.tex <==

\section{Method}




%\section{GnorNets}
%
%Attention span is defined as a linear combination of attention units, divided by the number of social media accounts with poorly configured notification settings.
%
%is bliss. Denoising/ distracting encoder (a special case of the noising encoder).  We provide a tractable approximation to the theoretical optimal solution (a constant time algorithm).  Random features may still contain information...
%
%
%G-Unit \footnote{We note that \textit{The Game} would also make a good choice here - it's a matter of taste.}.
%
%
%Two component model for \textit{visual attention} - bottom up saliency, top down task specific control.  Retinal pathway.
%
%GnorNets can be constructed from their constituent GnorUnits by combining the community best practices of neural network design with the ability to deliver a strong Jenga endgame under pressure (cf. \cite{scott2006jenga}).
%
%Disinterestedness score is given by one minus the dot product (in self attn).
%
%Learning is conducted by transforming the inputs on a \textit{need to know} basis (a basis of need-to-knows).
%
%Metaphor as a stagelight in classic neuro paper.
%
%Section on interpretability.

%
%Under the Generative Unadversarial Network framework, we simultaneously train
%two models: a generator $G$ that does its best to capture whichever data 
%distribution it feels it can manage and a motivator $M$ that helps $G$ to 
%achieve its dream. The generator is trained by learning a function 
%$G(\vec{z};\theta_g)$ which transforms samples from a uniform prior 
% distribution $p_z(\vec{z})$ into the space graciously accommodating 
% the data\footnote{The choice of the uniform prior prevents discrimination 
% against prior samples that lie far from the mean. It's a small thing, 
% but it speaks volumes about our inclusive approach.}.  The motivator is 
% defined as a function $M(\vec{x};\theta_M)$ which uses gentle gradients
% and persuasive language to encourage $G$ to improve its game.  In particular,
% we train $G$ to maximise $log(M(G(\vec{z}))$ and we simultaneously train 
% $M$ to maximise $log(M(G(\vec{z}))$. Thus, we see that the objectives of 
% both parties are aligned, reducing conflict and promoting teamwork.
% 
%
%
%The core components of our framework are illustrated in Figure 
%\ref{fig:training}. The GUN training scheme was inspired largely by Clint 
%Eastwood's memorable performance in \textit{Dirty Harry} but also in part by 
%the Transmission Control Protocol (TCP) three-way handshake 
%\citep{postel1981transmission}, which was among the first protocols to build 
%harmony through synergy, acknowledgements and the simple act of shaking hands.
%A description of the training procedure used to train $G$ and $M$ is given in 
%Algorithm \ref{trainingAlgo}. 
% 
% \begin{figure}[t]
%    \centering
%    \includegraphics[width=.9\textwidth]{figures/distributions.png}
%    \caption{(a) GUNs are trained by updating the generator distribution $G$ 
%    (yellow line) with the help and support of the motivator (red line) to 
%    reach its dream of the data distribution (blue dashed). (b) With a 
%    concerted effort, the generator reaches its goal. (c) Unlike previous 
%    generators which were content with simply reaching this goal, our generator 
%    is more motivated and gives it `$110\%$' moving it a further $10\%$
%    past the data distribution. While this isn't terribly helpful from a 
%    modelling perspective, we think it shows the right kind of attitude. 
%    }
%    \label{fig:mesh1}
%\end{figure}
%
% 
%\begin{algorithm}[t]
%  \caption{Training algorithm for Generative Unadversarial Networks}
%  \label{trainingAlgo}
%  \begin{algorithmic}[1]
%    \Procedure{Train}{}
%    \For{\texttt{\#iterations}}
%        \State Sample $n$ noise samples from prior $p_z(\vec{z})$ and compute 
%        $G({\vec{z}^{(1)};\theta_g), ...G({\vec{z}^{(n)};\theta_g)}}$.
%        \State Sample $n$ data samples ${\vec{x}^{(1)}, ...\vec{x}^{(n)},}$ 
%        from the data distribution.
%        \State Let $G$ show pairs 
%        $({\vec{x}^{(i)}}, G({\vec{z}^{(i)};\theta_g)})$ to $M$ as slides of a 
%        powerpoint presentation\footnotemark.        
%        \State Sample constructive criticism and motivational comments from $M$.
%        \State Update the powerpoint slides and incorporate suggestions into 
%        $\theta_G$.
%      \EndFor
%    \EndProcedure
%  \end{algorithmic}
%\end{algorithm} 
%\footnotetext{To guarantee polynomial runtime, it is important to ensure that the 
%generator is equipped with the appropriate dongle and works through any 
%issues with the projector \textit{before} the presentation begins.}
%
%Algorithm \ref{trainingAlgo} can be efficiently implemented by combining 
%a spare meeting room (which must have a working projector) and a top notch 
%deep learning framework such as MatConvNet \citep{vedaldi2015matconvnet} or 
%Soumith Chintala (Chintala, 2012-present).   We note that we can further 
%improve training efficiency by trivially rewriting our motivator objective 
%as follows\footnote{If this result does not jump out at you immediately, 
%read the odd numbered pages of \citep{amari2000methods}
%. This book should be read in Japanese. The 
%even-numbered pages can be ripped out to construct beautiful \emph{orizuru}.}:
%
%\begin{equation}
%    \theta_{M}^* = \underset{\theta_{M}}{\min} \oint\limits_{S(G)}\log(R) + \log(1-\zeta)
%    \label{eqn:loss}
%\end{equation}
%
%Equation \ref{eqn:loss} describes the flow of reward and personal 
%well-being on the generator network surface. $\zeta$ is a constant which 
%improves the appearance of the equation.  In all our experiments, we fixed 
%the value of $\zeta$ to zero.

\pagebreak

